WeAct: Dynamic Weight Switching as Agent Actions

Long-horizon agents must learn heterogeneous capabilities from interleaved trajectories. Updating shared parameters to learn new capabilities can degrade previously acquired ones, resulting in catastrophic forgetting. As a trajectory unfolds, different stages may require different capabilities, yet conventional joint training and static adapter merging maintain a fixed parameter configuration throughout execution. We introduce WeAct (Weight-level Internal Actions), which trains independent capability-specific LoRA adapters over a frozen backbone and adds adapter selection to the agent's action space. These internal actions use the model's native tool-calling interface for on-demand capability composition in a shared context. Across eight deep-research benchmarks, Qwen3-32B with WeAct improves average accuracy by 6.2% relative to full fine-tuning counterparts despite using less compute, and by 27.5% relative to the strongest static LoRA-merging method. WeAct also supports modular continual adaptation, by adding a new code computation adapter to expand the agent's capabilities and updating the existing writing adapter to improve report quality. Both updates leave the backbone and other adapters unchanged, supporting modular continual adaptation in agents.

==> Figures/03-capability-separation/learning/capability-retention-caption.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.8\linewidth]{Figures/03-capability-separation/learning/capability-retention.pdf}
\caption{\textbf{Retention under sequential capability training.}
(a)~Acquired accuracy gain lost, pooled over the four orders where each capability precedes another.
(b)~Orders in which \emph{both} earlier capabilities retain the required share of their gains. Both partitioned libraries contain
three rank-32 adapters. Fixed routes, one seed, balanced training, 168 test trajectories; details in
Appendix~\ref{app:sequential-retention}.}
\label{fig:capability-retention}
\end{figure*}


==> Figures/03-capability-separation/learning/capability-retention-recovery-caption.tex <==
\begin{figure}[!htbp]
\centering
\centering
\includegraphics[width=\linewidth]{Figures/03-capability-separation/learning/capability-retention-recovery.pdf}
\caption{\textbf{Replay cost of recovering earlier gains.} Ten matched cases with a 99\% monitoring-set target. Shared ranks are 8/24; partitioned libraries use three rank-8 adapters.}
\label{fig:capability-retention-recovery}
\end{figure}


==> Figures/03-capability-separation/static-fusion/merge-nll-gap.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{Figures/03-capability-separation/static-fusion/claim1_capability_gap.pdf}
\caption{Target-token NLL increase under static fusion relative to the capability-matched Individual adapter. Bars show record-mean paired differences; zero denotes equal target-text fit. Error bars are 95\% trajectory-bootstrap confidence intervals.}
\label{fig:merge-nll-gap}
\end{figure*}


==> Tables/1-table.tex <==
\begin{table*}[t]
\centering
\caption{[Placeholder - replace by image, not table] Comparison of capability injection methods for LLM agents. \method performs action-level weight reconfiguration without a learned router or base-model modification.\sz{table is hard to read, need to consistently check the row/column name}}
\label{tab:comparison}
% \setlength{\tabcolsep}{2.5pt}
\scriptsize
\begin{tabular}{@{}l C{1.35cm} C{1.2cm} C{1.45cm} C{1.35cm} C{1.3cm} C{1.45cm} C{1.5cm}@{}}
\toprule
& \textbf{Full SFT/RL}
& \textbf{Single LoRA}
& \textbf{Static Merge} \newline {\tiny DARE/TIES}
& \textbf{Token MoE} \newline {\tiny METeoRA}
& \textbf{Multi-Agent}
& \textbf{Prompt-as-Skill}
& \textbf{\method} \newline {\tiny Ours} \\
\midrule
\multicolumn{8}{@{}l}{\textsc{Architecture}} \\[1pt]
Injection
  & Full params & Low-rank & Low-rank & Low-rank & Full $\times N$ & Input (ctx) & Low-rank \\
Granularity
  & None & None & None & Per token & Per call & Per load & Per action \\
Shared ctx?
  & --- & --- & --- & Yes & No & Yes & Yes \\
\midrule
\multicolumn{8}{@{}l}{\textsc{Training \& Deployment}} \\[1pt]
Base mod.?
  & Yes (all) & No & No & Yes (gate) & Yes $\times N$ & No & No \\
Router?
  & --- & --- & --- & Required & --- & None & None (tool-call) \\
Extensibility
  & Retrain all & Retrain LoRA & Retrain +merge & Retrain gate & Deploy agent & Add prompt & Train +register \\
\midrule
\multicolumn{8}{@{}l}{\textsc{Capability \& Robustness}} \\[1pt]
Forgetting
  & Severe & Mild & Mild--mod. & Mild (drift) & Per-agent & Zero & Zero \\
Ctx.\ cost
  & None & None & None & None & $N\!\times\!$full & High & Minimal \\
Scaling
  & Conflict$\uparrow$ & 1-adapt.\ lim. & Interf.$\uparrow$ & Moderate & Coord.\ cost & Ctx.\ overflow & Linear \\
Interpretability
  & Black box & Black box & Black box & Opaque & Agent-lvl\sz{what does lvl stand for?} & Skill-lvl & Action-lvl \\
\midrule
\multicolumn{8}{@{}l}{\textsc{Cost}} \\[1pt]
Build
  & High & Med & Med+ & High & High$\times N$ & Low & Med \\
Infer.\ overhead
  & None & Minimal & None & Gate comp. & $N\!\times\!$infer. & Extra tok. & Swap \\
\bottomrule
\end{tabular}
\end{table*}

==> Tables/2-table.tex <==
\begin{table}[t]
\centering
\fontsize{10}{12}\selectfont
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\linewidth}{@{}cl>{\raggedright\arraybackslash}X@{}}
\toprule
\textbf{Turn} & \textbf{Label} & \textbf{Agent action (abbreviated)} \\
\midrule
1 & \texttt{plan} & ``The question requires comparing two claims. I will first search for source A, then source B, then cross-check.'' \\
2 & \texttt{search} & \texttt{web\_search("claim A evidence")} \\
3 & \texttt{search} & Reads the returned sources and extracts the relevant dates. \\
4 & \texttt{search} & Compares extracted dates against the original claim; identifies a discrepancy. \\
5 & \texttt{writing} & Produces the final answer with supporting evidence. \\
\bottomrule
\end{tabularx}
\caption{Illustrative capability labels for a trajectory segment. Each row is one assistant turn; labels follow the stage's function.}
\label{tab:span-example}
\end{table}


==> Tables/RQ2-budget-sweep.tex <==
\begin{table}[t]
\centering
\caption{Budget-sweep diagnostic on held-out \dataset{WebWalkerQA}. Tool-call caps are varied while generated-token and assistant-turn caps are held fixed at the matched-budget setting.\captionplaceholder}
\label{tab:rq2-budget-sweep}
\vspace{0.2em}
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lccc@{}}
\toprule
Method & 8 tools & 16 tools & 24 tools \\
\midrule
Single LoRA & 42.0\placeholder & 50.2 & 52.8 \\
Single LoRA, $3r$ & 42.5\placeholder & 51.0 & 54.1 \\
Full SFT & 41.8\placeholder & 49.7 & 57.6 \\
\method-hard & 49.3\placeholder & 57.5 & 59.2 \\
\method-soft & 48.4\placeholder & 56.3 & 58.4 \\
\bottomrule
\end{tabular}
\vspace{-0.8em}
\end{table}


==> Tables/RQ2-full-efficiency.tex <==
\begin{table}[t]
\centering
\caption{Full trajectory statistics on held-out \dataset{WebWalkerQA}. Source utilization measures the fraction of retrieved unique sources that are cited or used in the final answer.\captionplaceholder}
\label{tab:rq2-full-efficiency}
\vspace{0.2em}
\scriptsize
\setlength{\tabcolsep}{2.7pt}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
Method & Final $\uparrow$ & Gen. tok. $\downarrow$ & Tools $\downarrow$ & Turns $\downarrow$ & Unique src. & Src. util. $\uparrow$ & Dup. query $\downarrow$ & Model-sec. $\downarrow$ \\
\midrule
Single LoRA & 52.8\placeholder & 12.4k & 14.8 & 20.5 & 8.4 & 0.46 & 0.19 & 38.0 \\
Single LoRA, $3r$ & 54.1\placeholder & 13.2k & 15.1 & 21.3 & 8.8 & 0.47 & 0.18 & 39.3 \\
Full SFT & 57.6\placeholder & 18.9k & 24.7 & 31.5 & 11.9 & 0.43 & 0.24 & 51.2 \\
\method-hard & 59.2\placeholder & 13.7k & 15.4 & 22.0 & 10.6 & 0.58 & 0.12 & 41.2 \\
\method-soft & 58.4\placeholder & 14.2k & 16.1 & 22.8 & 10.4 & 0.55 & 0.13 & 42.4 \\
\bottomrule
\end{tabular}
\vspace{-0.8em}
\end{table}


==> Tables/RQ2-main-efficiency.tex <==
\begin{table}[t]
\centering
\caption{Trajectory-efficiency summary on held-out \dataset{WebWalkerQA} trajectories. ``Matched'' reports the score under common generated-token, external-tool-call, and assistant-turn caps across methods.\captionplaceholder}
\label{tab:rq2-main-efficiency}
\vspace{0.2em}
\scriptsize
\setlength{\tabcolsep}{3.2pt}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Final $\uparrow$ & Gen. tok. $\downarrow$ & Tools $\downarrow$ & Turns $\downarrow$ & Score / 1k tok. $\uparrow$ & Matched $\uparrow$ \\
\midrule
Single LoRA & 52.8\placeholder & 12.4k & 14.8 & 20.5 & 4.26 & 49.6 \\
Single LoRA, $3r$ & 54.1\placeholder & 13.2k & 15.1 & 21.3 & 4.10 & 50.4 \\
Full SFT & 57.6\placeholder & 18.9k & 24.7 & 31.5 & 3.05 & 51.8 \\
\rowcolor{red!5}
\method-hard & 59.2\placeholder & 13.7k & 15.4 & 22.0 & 4.32 & 57.9 \\
\rowcolor{orange!8}
\method-soft & 58.4\placeholder & 14.2k & 16.1 & 22.8 & 4.11 & 56.7 \\
\bottomrule
\end{tabular}
\vspace{-0.8em}
\end{table}


==> Tables/RQ2-system-cost.tex <==
\begin{table}[t]
\centering
\caption{System-cost statistics for the RQ2 latency analysis. The preload--retain row is the intended deployment setting, while recompute is a correctness-sensitive cache policy reference.\captionplaceholder}
\label{tab:rq2-system-cost}
\vspace{0.2em}
\scriptsize
\setlength{\tabcolsep}{3.0pt}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Mode & Preload & KV policy & Switches & Total sec. $\downarrow$ & Switch sec. $\downarrow$ & Extra VRAM \\
\midrule
Single LoRA & yes & retain & 0.0 & 54.9\placeholder & -- & 1.0$\times$ \\
Single LoRA, $3r$ & yes & retain & 0.0 & 57.5\placeholder & -- & 2.8$\times$ \\
Full SFT & -- & retain & 0.0 & 82.7\placeholder & -- & full model \\
\method preload & yes & retain & 5.4 & 62.6\placeholder & 0.4 & 3.1$\times$ \\
\method cold-load & no & retain & 5.4 & 74.2\placeholder & 2.9 & 1.1--3.1$\times$ \\
\method preload & yes & recompute & 5.4 & 73.0\placeholder & 0.5 & 3.1$\times$ \\
\bottomrule
\end{tabular}
\vspace{-0.8em}
\end{table}


==> Tables/cache-validity.tex <==
\definecolor{baseGray}{RGB}{178,178,178}
\definecolor{prevCyan}{RGB}{75,165,189}
\definecolor{activeRed}{RGB}{196,71,55}
\definecolor{refillPink}{RGB}{236,151,151}

% --- inline cache-bar primitives -------------------------------------------

\providecommand{\cbh}{1}
\providecommand{\cbfill}[3]{\draw[fill=#3, draw=black!45] (#1,0) rectangle +(#2,\cbh);}
\providecommand{\cbhatch}[2]{\draw[pattern=north east lines,
  pattern color=black!75, draw=black!45] (#1,0) rectangle +(#2,\cbh);}
\providecommand{\cbsbase}[2]{\cbfill{#1}{#2}{baseGray}}
\providecommand{\cbsbasestale}[2]{\cbfill{#1}{#2}{baseGray}\cbhatch{#1}{#2}}
\providecommand{\cbsprev}[2]{\cbfill{#1}{#2}{prevCyan}}
\providecommand{\cbsprevstale}[2]{\cbfill{#1}{#2}{prevCyan}\cbhatch{#1}{#2}}
\providecommand{\cbsrefill}[2]{\cbfill{#1}{#2}{refillPink}}
% \cachebar{state of base context}{state of prev.\ span}{state of later obs.}
\providecommand{\cachebar}[3]{%
  \begin{tikzpicture}[x=0.0438cm, y=0.24cm, baseline=-0.35ex]
    \csname cbs#1\endcsname{0}{34}%
    \csname cbs#2\endcsname{34}{12}%
    \csname cbs#3\endcsname{46}{14}%
    \draw[dashed, black!60, line width=0.3pt] (62,-0.3) -- (62,1.3);
    \cbfill{64}{11.5}{activeRed}%
  \end{tikzpicture}}
% Legend swatches, sized to sit on a text line.
\providecommand{\cbkey}[1]{%
  \begin{tikzpicture}[baseline=-0.35ex]
    \draw[fill=#1, draw=black!45] (0,0) rectangle (0.9em,0.62em);
  \end{tikzpicture}}
\providecommand{\cbkeystale}{%
  \begin{tikzpicture}[baseline=-0.35ex]
    \draw[fill=white, draw=black!45] (0,0) rectangle (0.9em,0.62em);
    \draw[pattern=north east lines, pattern color=black!75, draw=black!45]
      (0,0) rectangle (0.9em,0.62em);
  \end{tikzpicture}}

\begin{table}[t]
\centering
\caption{Adapter architecture $\times$ cache policy on held-out
\dataset{WebWalkerQA}. The last column draws the mechanism behind each
row: the bar runs over the trajectory prefix at a switch---task
context, the span generated under the previous adapter, later
observations---then, after the dashed line, generation under the active
adapter. Fill colour is the weight state that produced the cached
entries, so hatched area locates the approximation and pink width is
what removing it costs. Rows 1--2 price the approximation the main
comparison relies on; rows 3--4 price the one that survives inside
gating.\captionplaceholder}
\label{tab:cache-validity}
\vspace{0.2em}
\centerline{\scriptsize
  \cbkey{baseGray}~base-processed\quad
  \cbkey{prevCyan}~prev.\ adapter\quad
  \cbkey{refillPink}~(re-)prefilled at switch\quad
  \cbkey{activeRed}~active adapter\quad
  \cbkeystale~stale for the active adapter}
\vspace{0.45em}
\scriptsize
\setlength{\tabcolsep}{2.9pt}
\begin{tabular}{@{}llccccc@{}}
\toprule
Adapter & Cache policy & Reuse semantics & Score $\uparrow$
& \makecell[c]{TTFT after\\switch (s) $\downarrow$}
& \makecell[c]{Total\\sec. $\downarrow$}
& Cache state at switch \\
\midrule
\rowcolor{red!5}
Standard & retain (deployed) & approximate
  & 59.2\placeholder & \placeholder & 62.6\placeholder
  & \cachebar{basestale}{prevstale}{basestale} \\
Standard & recompute & exact
  & \placeholder & \placeholder & 73.0\placeholder
  & \cachebar{refill}{refill}{refill} \\
\midrule
\rowcolor{orange!8}
Gated & retain & exact on base spans
  & \placeholder & \placeholder & \placeholder
  & \cachebar{base}{prevstale}{base} \\
Gated & re-prefill prior spans & exact end to end
  & \placeholder & \placeholder & \placeholder
  & \cachebar{base}{refill}{base} \\
\bottomrule
\end{tabular}
\vspace{-0.8em}
\end{table}


==> Tables/capability-retention-controls.tex <==

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\caption{Matched sequential and interleaved controls at ranks 8/24: final content-token accuracy (\%). Both partitioned libraries contain three rank-8 adapters. Sequential results average all three capabilities and all six orders; the range is across order means, not an uncertainty interval. The unfinished random-partition interleaved run is marked pending. All rows use one seed and 168 test trajectories.}
\label{tab:retention-schedule-controls}
\begin{tabular}{lrrr}
\toprule
Adapter organization & Sequential & Interleaved & Order range (pp) \\
\midrule
Single-LoRA (rank 8) & 86.22 & 87.21 & 0.76 \\
Single-LoRA (rank 24) & 86.16 & 87.26 & 0.77 \\
Random partition & 85.75 & Pending & 0.44 \\
Capability adapters & 87.11 & 87.07 & 0.07 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/capability-retention.tex <==

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\caption{Absolute and relative loss of acquired content-token accuracy. Both partitioned libraries contain three rank-32 adapters. Each capability is averaged over the four orders in which it precedes another capability, using all 168 test trajectories. Acquired and lost gains are in percentage points; the final column is the ratio of the unrounded means. Balanced exposure, one training seed.}
\label{tab:capability-retention}
\begin{tabular}{llrrr}
\toprule
Adapter organization & Capability & Acquired & Lost & Lost (\%) \\
\midrule
Single-LoRA (rank 32) & Plan & 14.28 & 1.67 & 11.7 \\
 & Search & 6.95 & 1.57 & 22.6 \\
 & Writing & 3.05 & 1.41 & 46.2 \\
\addlinespace
Single-LoRA (rank 96) & Plan & 14.31 & 1.82 & 12.7 \\
 & Search & 6.81 & 1.68 & 24.7 \\
 & Writing & 3.06 & 1.50 & 49.2 \\
\addlinespace
Random partition & Plan & 13.36 & 1.32 & 9.9 \\
 & Search & 6.16 & 0.96 & 15.6 \\
 & Writing & 2.58 & 1.09 & 42.4 \\
\addlinespace
Capability adapters & Plan & 14.22 & 0.00 & 0.0 \\
 & Search & 6.84 & 0.00 & 0.0 \\
 & Writing & 3.09 & 0.00 & 0.0 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/cost-map.tex <==

\begin{table}[t]
\centering
\caption{Where each adaptation regime pays for heterogeneity.
Difficulty does not disappear under reparameterization; it moves.
Monolithic training pays at \emph{training time} (interference,
capacity), static fusion pays at \emph{inference time} (fusion
residual on every token), and dynamic selection pays a \emph{control}
cost (routing regret, switching overhead) that
Secs.~\ref{sec:exp:routing-ladder}--\ref{sec:exp:rq2-efficiency} show
is small and bounded.}
\label{tab:cost-map}
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lccccc@{}}
\toprule
& \makecell[c]{Training\\interference}
& \makecell[c]{Fusion\\residual}
& \makecell[c]{Capacity\\pressure}
& \makecell[c]{Routing\\regret}
& \makecell[c]{Zero-drift\\state} \\
\midrule
Full SFT / Single LoRA & \textbf{high} & --- & \textbf{high} & --- & none \\
Static merge (TIES/DARE) & low & \textbf{high} & med & --- & none \\
\method (dynamic selection) & low & 0 on active span & low & small (\S\ref{sec:exp:routing-ladder}) & offload $=$ base \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/merge-residual.tex <==

\begin{table}[t]
\centering
\caption{Fusion residual $\mathrm{Res}_k$ per capability and pairwise
principal angles after static merging of the trained
\texttt{plan}/\texttt{search}/\texttt{writing} adapters
(Sec.~\ref{sec:exp:static-fusion}). Dynamic selection zeroes the
active-span residual by construction. Entries are planned
measurements.}
\label{tab:merge-residual}
\scriptsize
\providecommand{\tbd}{}\renewcommand{\tbd}{\textcolor{gray}{\textemdash}}
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Merge method}
& $\mathrm{Res}_{\texttt{plan}}\downarrow$
& $\mathrm{Res}_{\texttt{search}}\downarrow$
& $\mathrm{Res}_{\texttt{writing}}\downarrow$
& \makecell[c]{Target Avg.\,$\uparrow$} \\
\midrule
Linear merge            & \tbd & \tbd & \tbd & \tbd \\
TIES-Merging            & \tbd & \tbd & \tbd & \tbd \\
DARE                    & \tbd & \tbd & \tbd & \tbd \\
Dynamic selection (\method) & \multicolumn{3}{c}{0 on active span (by construction)} & \tbd \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/routing-ladder.tex <==

\begin{table}[t]
\centering
\caption{Routing ladder on the fixed \texttt{plan}/\texttt{search}/\texttt{writing} library.
Each rung changes only \emph{how} adapters are invoked. The random
controls isolate raw adapter capacity and switch count from
\emph{semantic} selection; the query-level rung
(LoRA-as-Tools~\citep{adaptiveminds}) routes once per query and never
switches within a trajectory. Oracle--soft gap is reported as routing
regret. Entries marked ``\textcolor{gray}{\textemdash}'' are planned
runs.}
\label{tab:routing-ladder}
\scriptsize
\setlength{\tabcolsep}{4pt}
\providecommand{\tbd}{}\renewcommand{\tbd}{\textcolor{gray}{\textemdash}}
\begin{tabular}{@{}lccrrr@{}}
\toprule
\textbf{Routing policy} & \makecell[c]{Semantic\\selection?} & \makecell[c]{In-trajectory\\switching?}
& \makecell[c]{Target\\Avg.\,$\uparrow$} & \makecell[c]{Oracle\\agreement\,$\uparrow$} & \makecell[c]{Switches\\/traj.} \\
\midrule
always-base (no adapters)        & ---           & ---          & \tbd & --- & 0 \\
always-on best single adapter    & ---           & $\times$    & \tbd & --- & 0 \\
random per-trajectory            & $\times$     & $\times$    & \tbd & \tbd & 0 \\
random switching (matched count) & $\times$     & \checkmark    & \tbd & \tbd & \tbd \\
frequency-prior switching        & weak          & \checkmark    & \tbd & \tbd & \tbd \\
query-level routing (LoRA-as-Tools) & \checkmark  & $\times$    & \tbd & \tbd & 0 \\
\midrule
\method-hard (workflow)          & rule          & \checkmark    & \tbd & \tbd & \tbd \\
\method-soft (self-routing)      & \checkmark     & \checkmark    & \tbd & \tbd & \tbd \\
\method-soft (oracle)            & perfect       & \checkmark    & \tbd & 100  & \tbd \\
\bottomrule
\end{tabular}
\end{table}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

